Rigorous Analysis of Software Countermeasures against Cache Attacks

CPU caches introduce variations into the execution time of programs that can be exploited by adversaries to recover private information about users or cryptographic keys. Establishing the security of countermeasures against this threat often requires intricate reasoning about the interactions of program code, memory layout, and hardware architecture and has so far only been done for restricted cases. In this paper we devise novel techniques that provide support for bit-level and arithmetic reasoning about memory accesses in the presence of dynamic memory allocation. These techniques enable us to perform the first rigorous analysis of widely deployed software countermeasures against cache attacks on modular exponentiation, based on executable code.

==> Makefile <==
TEX = pdflatex -shell-escape -interaction=nonstopmode -file-line-error
PRE =  $(TEX) -ini -job-name="preamble" "&pdflatex preamble.tex\dump"
BIB = bibtex
EXECUTABLE = main.pdf

.PHONY: all view

BIBFILES=$(wildcard *.bib)
TEXFILES=$(wildcard *.tex)

all : $(EXECUTABLE)

$(EXECUTABLE) : $(TEXFILES) main.bbl main.blg
	$(TEX) main.tex

main.bbl main.blg : $(BIBFILES)
	$(BIB) main

# main.aux : main.tex
# 	$(TEX) main.tex

# $(BIBFILES) : main.tex
# 	$(TEX) main.tex


==> meld <==
Index: obsdomains.tex
===================================================================
--- obsdomains.tex	(revision 516)
+++ obsdomains.tex	(working copy)
@@ -22,7 +22,7 @@
 \subsection{Representation}
 \TODO{Take offsets out of masked symbols.}
 The masked symbol domain is based on finite sets of what we call {\em
-  masked symbols}, which are pairs $(\constsym,\mask,\offset)$ consisting of 
+  masked symbols}, which are pairs $(\constsym,\mask)$ consisting of 
 the following components:
 {\em symbol} $\constsym\in \Cons$, uniquely 
 identifying an unknown value, 
@@ -29,11 +29,9 @@
 such 
 as a base address; a {\em mask}
 $\mask \in\{0,1,\top\}^\bitlen$, representing a pattern of known and unknown 
-bits; and an {\em offset}
-$\offset\in\{0,1\}^\bitlen$, representing an offset from the unknown
 bits.
 The $i$-th bit of a masked symbol
-$(\constsym,\mask,\offset)$ is equal to $\mask_i\in\{0,1\}$, unless
+$(\constsym,\mask)$ is equal to $\mask_i\in\{0,1\}$, unless
 $\mask_i=\top$, in  which case it is unknown.
 In the first case we call
 the bit {\em masked}, in the second {\em symbolic}. We abbreviate the
@@ -42,8 +40,8 @@
 
 Two special cases are worth pointing out:
 \begin{compactenum}
-\item $(\constsym,\top,0)$ represents an unknown value, and
-\item $(\constsym,\mask,0)$ with $\mask\in\{0,1\}^\bitlen$ represents the
+\item $(\constsym,\top)$ represents an unknown value, and
+\item $(\constsym,\mask)$ with $\mask\in\{0,1\}^\bitlen$ represents the
 bit-vector $\mask$.
 \end{compactenum}
 % That is, pairs of the form $(\constsym,\mask,\offset)$ generalize both
@@ -61,9 +59,9 @@
 $\symbmapping\colon \Cons\rightarrow \{0,1\}^\bitlen$ taking symbols to
 bit-vectors:
 \begin{equation*}
-  \conc_\symbmapping(F)=\{(\symbmapping(\constsym) \maskop \mask) + \offset
+  \conc_\symbmapping(F)=\{\symbmapping(\constsym) \maskop \mask
 \mid
-(\constsym,\mask,\offset) \in F\}\ .
+(\constsym,\mask) \in F\}\ .
 \end{equation*}
 Here $\maskop$ is defined bitwise by $(\symbmapping(\constsym))_i\maskop 
 m_i=m_i$ if
@@ -95,6 +93,15 @@
   projection $\view$ mapping vectors to a subset of their components, we have
   $\sizeof{\view(\conc_\symbmapping(F))}\le \sizeof{\view(F)}$.
 \end{proposition}
+\begin{proof}
+ (1) We have $\view(\conc_\symbmapping(F))=\conc_\symbmapping(view(F))$ because 
+$\view$ is a projection and $\conc_\symbmapping$ concretizes masked symbols 
+component-wise.
+(2) We have |gamma(view(F))|<=|view(F)| because the range of any function is at 
+most as large as its domain.  Hence, we have |view(gamma(F))|<=|view(F)|.
+\end{proof}
+
+
 Proposition~\ref{prop:quant} gives a means to bound the
 range of the adversary's view, for {\em any} valuation of
 the symbols.
@@ -116,22 +123,7 @@
 % blocks (and if we have $s+65$, 
 % it will lie in a third one).}
 
-\TODO{This example is wrong. Remove it.}
-  \begin{example}[Offsets]
-  The projection of the set 
- \\$
-F=\{(s,\top,(1,0,0)), (s,\top,(1,0,1)), (s,\top,(1,1,0))\}
-$
-of (three bit) masked symbols
-to their least significant bit yields the set $\{(s_0 + 0), (s_0 + 1)\}$, i.e., 
-we
-count two observations. The projection to their most
-significant bit yields only the singleton set $\{(s_2 + 1)\}$, i.e., the
-cardinality is determined to be $1$ without the knowledge of the valuation of 
-$s$. 
-\end{example}
 
-
 The update of masked symbols ensures that whenever a bit is 
 masked, the offset-bit is~$0$, thus each bit from a masked symbol can be either 
 seen as a masked bit $m_i$, or as a symbol with an offset $s_i + o_i$. This 


==> observers.tex <==
\section{Capturing Memory Trace Observers}
This section: Technical contributions to capture the adversary models.

\TODO{Related: trace partitioning; there they do delayed joins.}

In this section we elaborate on the novel abstractions which we develop to 
capture memory trace observers (see Section~\ref{sec:hierarchy}).
\subsection{Trace DAG Representation}

To represent traces of addresses and blocks, we use a trace DAG abstraction, 
which compactly and precisely captures the set of traces, similar to the trace 
representation in~\cite{cacheaudit-tissec15}. The DAG has a 
dedicated root $r$ and a sink $s$, where initially $r = s$. The definition of 
the update and join functions make sure that at each point of the 
analysis there is only one sink, and for that reason we identify each DAG with 
the sink node. Each node $n\in N$ is labelled with a label 
$L(n)$, which represents the accessed address or memory block, depending on the 
observer. A path in the DAG represents a sequence of accessed addresses. 
Repeated accesses to the same address are represented as a single node, and we 
additionally maintain a value abstract domain $R$ to track the number of 
repetitions of each node, and $\gamma(R(n))$ represents the set of possible 
numbers of consecutive accesses to node $n$.
The domain $R$ can be implemented in a finite set or an interval abstraction.



In the trace DAG, the sink node $n$ represents the set of traces of the 
program until this point of the analysis, and its concretization function is 
defined as
$$\concFTraces(n) 
=\bigcup_{\substack{n_0\cdots n_k 
\text{ is a}\\ \text{path from $r$ to $n$}}}
\{\viewweakblockbound{\rangelower}{\rangeupper}(L(n_0)^{r_0}\cdots 
L(n_k)^{r_k}\mid r_i\in\concFTraces(R(n_i))\}$$


The trace abstraction is suited with two functions: an update and 
a join function. The trace update makes sure a new node is inserted only if the 
access is not repeated.
\[ \upd(n,a) =
  \begin{cases}
    n  &\quad \text{if $L(n) = \ell(n)$} \\
     n'      & 
\quad \text{otherwise ,}\\
  \end{cases}
\] 
where an edge $(n,n')$ is added, and $\ell(n)$ is an observer-specific 
labeling function. 
The repetitions-domain is updated accordingly, by incrementing 
the possible ages in $R(n)$ in the first case, and by adding 
the assignment $n' \mapsto \{1\}$ in the second case.


The join function is defined as follows:
\[ \joinfn(n_1,n_2) =
  \begin{cases}
    n_1  &\quad \text{if $n_1 = n_2$} \\
     \text{$n'$ }      & 
\quad \text{otherwise ,}\\
  \end{cases}
\] 
where $n'$ is a new node with parents $n_1,n_2$ and label $L(n')=\varepsilon$. 
While the second case applied to equal nodes represents the 
same set of concrete traces, establishing an equality of traces leads to a 
compacter representation, which also leads to more precision in the counting 
procedure described below. For b-block-traces, we achieve additional precision 
by delaying joins, as described in Section~\ref{sec:delay}.


The number of traces $\cnt(n)$ represented by the trace abstraction
 is the number of paths from $r$ to $n$, which we obtain by breadth-first 
search:
$$\cnt(n) = 
\sum\limits_{m\in\parents(n)}\mathit{num}_{(\rangelower,\rangeupper)}
(n)\cdot\cnt(m)\ .$$
Each node $n$ is counted according to the number of 
observations it $\mathit{num}$ it represents for the respective observer, as 
described below.

\subsection{Observer-specific Parameters}
Each of the observer types we represent by a dedicated trace abstraction, which 
differ in the $\ell$ and $\mathit{num}$ functions. For address-trace observers,
the labels are the accessed addresses themselves, i.e., $\ell(a) = a$. For the 
block- and b-block-trace observers, the nodes are labelled by the accessed 
block. For this, we
 define the $\abs{\blockfn}$-function which 
abstracts from the $\blockfn$-function by giving the same block identifier for 
addresses which the analysis can infer to share the same block, e.g. because 
they share the same most-significant bits. It is defined as
$$\abs{\blockfn}(a) = 
\begin{cases}
  \blockfn(a) & \quad \text{if $a\in\Cons\cup\Vars$} \\
  a         & \quad \text{otherwise\ ,} \\
\end{cases}
$$

The $\mathit{num}(n)$-function gives the number of observations node $n$ 
represents. For address- and block-trace observers, $\mathit{num}(n) = 
\sizeof{\gamma(R(n))}$. For b-block-trace observers, the number is $1$ if the 
observations are within the stuttering range:

$$
\mathit{num}_{(\rangelower,\rangeupper)}(n) = 
\begin{cases}
           1 & \text{if $n = r$} \\
           1 & \text{if } 
           \exists k\in \concFTraces(R(n)):k\in [\rangelower,\rangeupper]\\
           \cnt(\concFTraces(R(n))) & \text{otherwise}\\
          \end{cases}
$$

The soundness of the trace-abstractions follows directly from the definitions 
of the abstract update, because the abstract update coincides with the concrete 
update. Imprecisions however may come as a result of the imprecise counting 
procedure. In the following, we show how we eliminate such an imprecision for 
the b-block-trace observer, by enforcing a more compact DAG representation.

\subsection{Delayed Joins}\label{sec:delay}

In contrast to the address- and block-trace DAG, the b-block DAG may retain the 
same after an update function. This can lead to imprecise counting in case that 
$\upd(n_1,a) = \upd(n_2,a)$ when $n_1\neq n_2$, and we say that the DAGs 
$n_1,n_2$ have been collapsed to a single DAG. For example, this may happen if 
a $n_1 = b_1,b_2,b_3$, $n_2 = b_1,b_2$, and after joining $n_1$ and $n_2$, the 
block $b_3$ is accessed.

To gain precision, all joins $\joinfn(n_1,n_2)$ are delayed for one step  of 
the analysis, until
\begin{enumerate}[(i)]
 \item the next $\upd$ is applied; or
 \item the next $\joinfn$ is performed with an element $n_3\notin \{n_1,n_2\}$.
\end{enumerate}


In our analysis, we lay a particular value on precision in case the 
possible number of observation is $1$, i.e., the observer learns no 
information whatsoever. The following proposition shows that the one-step delay 
is optimal for detecting zero-leakage, i.e., delaying the join more than one 
step will not lead to better precision.

\begin{proposition}\label{prop:delay-optimality}
If after (i) or (ii) there is more than one distinct DAGs, performing further 
updates on the DAGs cannot collapse the DAGs to a single DAG.
\end{proposition}
\begin{lemma}\label{lem:sequences} Let $s,t$ be finite sequences of elements, 
and let ($b_1\concat b_2\concat  b_3\cdots$) be an infinite sequence 
of elements.
If $s\neq t$, then the concatenation of $s,t$ with $b_1\concat 
b_2\concat b_3\cdots$ results in 
  $$t\concat b_1\concat b_2\concat b_3\cdots \neq t\concat  
b_1\concat  
b_2\concat b_3\cdots$$
\end{lemma}


\begin{proof}[Proof of Proposition~\ref{prop:delay-optimality}]
Considering case (i), we have $n_1, n_2$, such that  $\upd(n_1, 
b)\neq\upd(n_2,b))$. Let $b_1\concat b_2\cdots$ be an infinite sequence 
of block addresses. To show is that $\upd(\upd(\upd(n_1,b),b_1),b_2),\dots\neq\\
\qquad\upd(\upd(\upd(n_2,b),b_1),b_2),\dots$.

After the first update, both DAGs 
are guaranteed to have the same label at the last node, however their 
inequality indicates that w.l.o.g. there is a path $p_1$ from $r$ to $n'_1$ 
which is not equal to any path from $r$ to $n'_2$, and thus $p_1\neq p_2$. 
Thus, according to Lemma~\ref{lem:sequences}, appending further nodes to $p_1$ 
or $p_2$ cannot make them equal.
% 
% \begin{enumerate}[(a)]
% \item One element is retained and one is changed, i.e., \\$\upd(n_1, b)=n_1$, 
% $\upd(n_2,b))= n'_2$. Then, there is are paths $(r,u_1,u_2,\dots,u_k,n_1)$ 
% and 
% $(r,v_1,v_2,\dots,v_k,n_2,n'_2)$, such that $L(n_1) = b = L(n'_2) 
% \neq L(n_2)$. Thus, the sequences $L(r)\concat L(u_1) \cdots L(u_k) \concat 
% L(n_1) \neq \\L(r)\concat L(v_1) \dots L(v_k)\concat L(n_2) \concat L(n'_2)$, 
% and according to Lemma~\ref{lem:sequences}, the statement holds.
% \item Both elements are retained, i.e., \\$\upd(n_1, b)=n_1$, $\upd(n_2,b))= 
% n_2$. Then, according 
%  \item Both elements are changed, i.e., $\upd(n_1, b)=n'_1$, $\upd(n_2,b)) = 
% n'_2$. % Then, $n_1 b \neq n_2 b$.
% 
% \end{enumerate}

\end{proof}


